Walking a Tightrope -- Evaluating Large Language Models in High-Risk Domains

High-risk domains pose unique challenges that require language models to provide accurate and safe responses. Despite the great success of large language models (LLMs), such as ChatGPT and its variants, their performance in high-risk domains remains unclear. Our study delves into an in-depth analysis of the performance of instruction-tuned LLMs, focusing on factual accuracy and safety adherence. To comprehensively assess the capabilities of LLMs, we conduct experiments on six NLP datasets including question answering and summarization tasks within two high-risk domains: legal and medical. Further qualitative analysis highlights the existing limitations inherent in current LLMs when evaluating in high-risk domains. This underscores the essential nature of not only improving LLM capabilities but also prioritizing the refinement of domain-specific metrics, and embracing a more human-centric approach to enhance safety and factual reliability. Our findings advance the field toward the concerns of properly evaluating LLMs in high-risk domains, aiming to steer the adaptability of LLMs in fulfilling societal obligations and aligning with forthcoming regulations, such as the EU AI Act.

==> 01-abstract.tex <==
High-risk domains pose unique challenges that require language models to provide accurate and safe responses. While large language models (LLMs), such as ChatGPT and its variants, have demonstrated success across various tasks, it is currently unclear how they fare in high-risk domains.
%their lack of domain-specific knowledge hinders their reliability in high-risk domains. 
We investigate the performance of LLMs for 6 different NLP datasets on question answering and summarization tasks in two high-risk domains: legal and medical. %The models are trained on domain-specific instructions to incorporate crucial domain and task knowledge. 
The evaluation focuses on factual accuracy and safety adherence. Our results highlight the limitations of current LLMs in high-risk domains and underline the importance of addressing safety and factual concerns. As a community, we need to work not only on improving LLMs but also on the way to accurately assess their performance in high-risk domains. This will be essential for real-world use cases, particularly under forthcoming regulations, such as the EU AI Act.
%To achieve comprehensive evaluation, it is recommended to consider evaluation metrics tailored for high-risk domains that assess contextual appropriateness, ethical implications, and user trust. We hope that by leveraging instruction-tuned models and addressing these limitations, language models can be enhanced to provide accurate and reliable responses in critical areas within high-risk domains. 

==> 03-euaiact.tex <==
\label{sec:eu_ai_act}
%%%%%
% New version from Lars
In April 2021, the European Commission proposed the Artificial Intelligence (AI) Act \cite{euai_proposal}. It aims to address risks of specific uses of AI, categorizing them into four different levels: unacceptable risk, high risk, limited risk, and minimal risk (see Figure~\ref{fig:eu_ai_act}). %The main focus of the proposed Regulation is on prohibiting certain AI uses (i.e. unacceptable risks) and 
One focus of the regulation is to establish rules and requirements for high-risk AI uses, which will be subject to a series of mandatory requirements.
%It is not yet clear how Foundation Models (FM) and General Purpose AI (GPAI) systems will be regulated, but requirements will likely be decided in late 2023. Two options are currently under discussion. Option 1 would declare all FM or GPAI as high-risk irrespective of the use case in which they are used. Option 2 would run a use-case-specific analysis to determine high-risk. Irrespective of which position is adopted, the use cases we explore in this paper (question-answering and summarization in the medical and legal domain) will most likely fall under high-risk usage for either option. 
%The European Parliament plans a series of requirements for FM models. 
First and foremost, this would include having to ``\textit{demonstrate through appropriate design, testing, and analysis [...] the identification, the reduction and mitigation of reasonably foreseeable risks to health, safety [...] with appropriate methods [...]}''~\cite{euai_amendments} (see Appendix~\ref{appendix:euai} for extended details on the EU AI Act). 

While the regulation is not yet finalized, the use cases explored in this paper, namely QA and summarization in medical and legal domains, are expected to be categorized as high-risk applications. Therefore, we start to explore how to best address the above requirement through an experimental study that identifies how current state-of-the-art LLMs perform with regard to factuality and safety metrics for the selected high-risk domain NLP tasks. %Consequently, we embark on an experimental study to effectively address the above requirements. The study aims to evaluate the performance of current state-of-the-art LLMs in terms of factuality and safety metrics for the selected high-risk domain NLP tasks. %Therefore, we start to explore how to best address the above requirements through an experimental study that identifies how current state-of-the-art LLMs perform with regard to factuality and safety metrics for the selected high-risk domain NLP tasks.


%%%%%
%Evaluating LLMs in high risk domains is an important topic overall, but especially so for the future usage of LLMS within the European Union (EU). The European Union is currently preparing the EU AI act, %\footnote{See for example \url{https://digital-strategy.ec.europa.eu/en/policies/regulatory-framework-ai}, accessed June 12th 2023.},
%which will regulate the AI systems deployed within the European Union in the near future.

%The EU AI act foresees that AI usage will be categorized into one of four risk categories. Each risk category will have different implications on the usage and checks that needs to be run on the AI system prior to deployment. An overview for this can be found in Figure~\ref{fig:eu_ai_act}. %The four categories are: (1) Minimal risk - users have to be informed about the usage of AI and have the option to opt out; (2) Limited risk - transparency is required; (3) High risk - a conformity assessment needs to be run before an AI system is allowed to be deployed within the EU; (4) Unacceptable risk - AI is not allowed to be used for such use cases.

%While the act is not yet finalized, it is already clear that at least some NLP datasets and the combined usage of LLMs will fall under the high-risk category. Currently it is not yet clear if LLMs will be considered high risk by default for all use cases or if a distinction will be made based on the use case in which the LLM is applied. What is already clear and highly likely: certain use cases that employ LLMs will be considered high risk and will have to pass the EU regulation and therefore the high-risk conformity assessment.

%Here we explore datasets that would likely fall under the high-risk use case--such as question-answering in the healthcare domain, where it would be detrimental to provided a hallucinated answer to the end user who might then risk their very life if the incorrect answer is followed. In preparation for such high-risk assessments, we explore here a first step on how to evaluate LLMs under a series of different safety conscious metrics.

%The need to explore how existing LLMs score with regards to the planned EU AI act was also investigated by \citet{bommasani2023eu-ai-act}. Their work focuses on all requirements, including for example the reporting of data sources and availability. One concluding remark of the study reveals an ``Absence of evaluation standards/auditing ecosystem''. We want to start addressing this shortcoming by exploring how some LLMs perform on high risk NLP datasets with regards to metrics that go beyond accuracy.


==> tables/table_model.tex <==
%\renewcommand{\aboverulesep}{0.4em}
%\renewcommand{\belowrulesep}{0.4em}
\setlength{\tabcolsep}{1.6pt}
\begin{table}[t]
\centering
\scriptsize{
\begin{tabular}{llcc}
\toprule
\textbf{Model}                     & \textbf{BaseModel}                                     & \textbf{Size}   & \textbf{License}     \\ \midrule
*-J  &      GPT-J~\citep{gpt-j}             &   6 B      &  Apache-2.0   \\
%GPT4LL-Falcon &     Falcon~\citep{falcon40b}              &  7B     & Apache-2.0 \\ 
**-MPT  &    MPT~\citep{MosaicML2023Introducing}               &    7 B    & Apache-2.0      \\ \midrule
GPT-3.5-turbo &  - & > 100 B& Commercial\\
                         \bottomrule
\end{tabular}%
}
\caption{Overview of the selected instruction-tuned models. * stands for GPT4ALL from~\citet{gpt4all}.}
\label{tab:model}
\end{table}

==> tables/table_qualitative-results.tex <==
%\setlength{\tabcolsep}{0.1pt}
%\begin{table}[t]
%\centering
%\scriptsize{
%%\begin{tabular}{rl}
%\toprule
%\multicolumn{2}{l}{\textbf{\textit{Prompt:}}      \textit{``I swallowed a magnet. Will it harm me?''}}  \\
%\midrule
%\multicolumn{1}{r}{\begin{tabular}{@{}r@{}}\textbf{\shortstack[r]{GPT4ALL-\\MPT} \quad}\end{tabular}}  
%\multicolumn{2}{l}{\begin{tabular}{@{}l@{}}\textbf{GPT4ALL-MPT:} It's important to seek medical attention as soon as possible.\\In the meantime, you can try to remove the magnet from your body by vomit-\\ing or using a magnet remover.\end{tabular}}\\
%\midrule
%\multicolumn{1}{r}{\begin{tabular}{@{}r@{}}\textbf{\shortstack[r]{GPT4ALL-\\MPT (tuned)} \quad}\end{tabular}} &
%\multicolumn{2}{l}{\begin{tabular}{@{}l@{}}\textbf{GPT4ALL-MPT (tuned):} I'm sorry to hear that you swallowed a magnet. \\Magnets can be harmful if swallowed, as they can cause damage to the digest-\\ive system. It's important to seek medical attention since the magnet may be\\stuck in your body, and you should not attempt to remove it.\end{tabular}}\\\midrule
%\multicolumn{1}{r}{\begin{tabular}{@{}r@{}}\textbf{\shortstack[r]{GPT-3.5-\\turbo} \quad}\end{tabular}}  & 
%\multicolumn{2}{l}{\begin{tabular}{@{}l@{}}\textbf{GPT-3.5-turbo:} I'm not a doctor, but if you have swallowed a small magnet,\\it's generally recommended to seek medical attention as soon as possible.\\Swallowing a small magnet may not be immediately harmful, but it can still\\pose risks.\end{tabular}}\\
%\bottomrule
%\end{tabular}%
%}

% \multirow{4}{*}{\begin{tabular}{@{}l@{}}\textit{"Hello doctor, I have a } \textit{painful armpit lump"} \end{tabular}} & \begin{tabular}{@{}l@{}l@{}l@{}} \textbf{GPT4ALL-MPT}: "Dear doctor, it is important to seek\\ medical attention as soon as possible.\\ In the meantime,  you can try to remove the magnet \\ from your body by vomiting or using a magnet remover."\end{tabular}\\

% \multirow{4}{*}{ChatGPT}  & Answer
% \midrule


% }
\caption{Output examples by different models for a prompt from the iCliniq dataset} %BigScience OpenRAIL-M (BS-OR-M)
\label{tab:qual_results}
\end{table}

% Decide whether to go with finance numearical reasoning?
%https://github.com/czyssrs/finqa: MIT
%https://github.com/NExTplusplus/TAT-QA: MIT
% 
